On the Vulnerability of Fairness Constrained Learning to Malicious Noise

We consider the vulnerability of fairness-constrained learning to small amounts of malicious noise in the training data. Konstantinov and Lampert (2021) initiated the study of this question and presented negative results showing there exist data distributions where for several fairness constraints, any proper learner will exhibit high vulnerability when group sizes are imbalanced. Here, we present a more optimistic view, showing that if we allow randomized classifiers, then the landscape is much more nuanced. For example, for Demographic Parity we show we can incur only a $\Theta(\alpha)$ loss in accuracy, where $\alpha$ is the malicious noise rate, matching the best possible even without fairness constraints. For Equal Opportunity, we show we can incur an $O(\sqrt{\alpha})$ loss, and give a matching $\Omega(\sqrt{\alpha})$lower bound. In contrast, Konstantinov and Lampert (2021) showed for proper learners the loss in accuracy for both notions is $\Omega(1)$. The key technical novelty of our work is how randomization can bypass simple "tricks" an adversary can use to amplify his power. We also consider additional fairness notions including Equalized Odds and Calibration. For these fairness notions, the excess accuracy clusters into three natural regimes $O(\alpha)$,$O(\sqrt{\alpha})$ and $O(1)$. These results provide a more fine-grained view of the sensitivity of fairness-constrained learning to adversarial noise in training data.

==> NeurIPS23/abstract.tex <==
\begin{abstract}

We consider the vulnerability of fairness-constrained learning to small amounts of malicious noise in the training data. \cite{lampert} initiated the study of this question and presented negative results showing there exist data distributions where for several fairness constraints, any proper learner will exhibit high vulnerability when group sizes are imbalanced. Here, we present a more optimistic view, showing that if we allow randomized classifiers, then the landscape is much more nuanced. For example, for Demographic Parity we show we can incur only a $\Theta(\alpha)$ loss in accuracy, where $\alpha$ is the malicious noise rate, matching the best possible even without fairness constraints. For Equal Opportunity, we show we can incur an $O(\sqrt{\alpha})$ loss, and give a matching $\Omega(\sqrt{\alpha})$ lower bound. In contrast, \cite{lampert} showed for proper learners the loss in accuracy for both notions is $\Omega(1)$. The key technical novelty of our work is how randomization can bypass simple "tricks" an adversary can use to amplify his power.  
We also consider additional fairness notions including Equalized Odds and Calibration. For these fairness notions, the excess accuracy clusters into three natural regimes $O(\alpha)$,$O(\sqrt{\alpha})$, and $O(1)$. These results provide a more fine-grained view of the sensitivity of fairness-constrained learning to adversarial noise in training data.

%We consider fairness-constrained ERM in the presence of  malicious noise \cite{malnoise}, where
%the adversary can corrupt a randomly sampled $\alpha$ fraction of the dataset.
  %in the setting of \cite{lampert}. 
 %\cite{lampert}shows undesirable excessive accuracy loss in this setting.
 %\pcomargincomment{I wonder if the previous sentence can be paraphrased, particularly the part "interpreting this..."}
  %  We consider a broader range of fairness notions and characterize the maximum accuracy loss 
   % when we allow a simple randomized classifer.
    %pcomargincomment{what does min-max mean here exactly? 
    %Is it like accuracy loss against worst-case adversary?} 
    %accuracy loss when we allow a simple  improper randomized classifier.
  
  %In particular, our work shows a more optimistic view than the impossibility results described in \cite{lampert}.
  %For Demographic Parity we attain the optimal $\Theta(\alpha)$ loss in accuracy and for Equal Opportunity $\Omega(\sqrt{\alpha})$ regardless of group size, in sharp contrast to\cite{lampert} where the loss in accuracy for both notions was $\Omega(1)$.
%  The key technical novelty of our work is how randomization weakens the ability of the adversary to use the fairness constraints to force poor classifier performance.
 
  %The key difference is we allow a randomized classifier created from a base hypothesis class that allows for smoothing out the power of the adversary. \pcocomment{what does smoothing out the power of the adversary mean?}
 %Additionally, we  consider a wide range of fairness notions including Demographic Parity, Equal Opportunity, Equalized Odds, Minimax fairness.
  %\ascomment{need to capitalize too?}, and a mix of Calibration notions. 
  %When considering these regimes, the excess accuracy clusters into three natural regimes $O(\alpha), O(\sqrt{\alpha}$, and $O(1)$.
  %These results provide a more fine-grained view of the sensitivity of Fair-ERM. 
  %78\pcomargincomment{I like this concluding sentence}
  %  At a high level our work shows that Fair ERM is as robust to malicious noise as plain ERM, assuming we have access to such a randomized classifier. 
  %For the range of fairness not
\end{abstract}

==> NeurIPS23/multigroup.tex <==
\subsection{ Multiple Groups}
\kmsmargincomment{I think this is all true but I need to think more closely---low priority since it can be done in the camera ready version}
In this paper, for ease of presentation we will focus on the disjoint case of binary groups i.e. two disjoint groups. 
Our core theorems have natural extensions to the case of an integer number of groups, where the adversary will typically attack the \emph{smallest group}.
%If the groups have non-empty intersection, this will not change the lower/upper bounds in this paper with the appropriate modification which we discuss in Appendix \ref{multgroup}.
\pcomargincomment{Is this actually true? It's not obvious to me that this holds. If a point lies in the intersection of A and B, how would the randomized classifier behave? which biased coin would they toss, the one for A or for B}
%In the case of group overlap, we can observe that our lower bounds depend on the size of the smallest group. 
The elegant and contemporary approach in \cite{multicalib} of defining relevant groups with a computationally rich class $C$ handles the issue of group and sub-group 
overlap \pcodelete{naturally}, %two naturals next to each other
but a natural research question is how that framework interacts with malicious noise and our closure model.
We briefly discuss this in Section \ref{sec:calib} as a direction for future research.
%but a full treatment of this important problem will be left for future research.


==> arxiv_style.tex <==
%\usepackage{geometry}
\usepackage[letterpaper, left=1in, right=1in, top=1in, bottom=1in]{geometry}

\usepackage[dvipsnames]{xcolor}
\usepackage[colorlinks=true, linkcolor=blue, citecolor=blue]{hyperref}
\usepackage{microtype}

% algorithms
%\usepackage{algorithm}
% \usepackage{algpseudocode}


\usepackage{natbib}
\bibliographystyle{plainnat}
\bibpunct{(}{)}{;}{a}{,}{,}

\usepackage{amsthm}
\usepackage{mathtools}
\usepackage{amsmath}
\usepackage{bbm}
\usepackage{amsfonts}
\usepackage{amssymb}
\let\vec\undefined
\usepackage{MnSymbol} %Actually conflicts with amssymb and others

\usepackage{xpatch}

%%% theorems

\theoremstyle{definition}  %Sets style of subsequent newtheorems to 'definition'
\newtheorem{assumption}{Assumption}
\newtheorem{claim}{Claim}
\newtheorem{exercise}{Exercise}
%\newtheorem{assumption}{Assumption}
\newtheorem{conjecture}{Conjecture}
\newtheorem{corollary}{Corollary}
\newtheorem{proposition}{Proposition}
\newtheorem{fact}{Fact}
\newtheorem{goal}{Goal}
%\newtheorem{model}{Model}
%\newtheorem{problem}{Problem}
\newtheorem{problem}{Problem}
\newtheorem{model}{Model}
\theoremstyle{plain}
\newtheorem{lemma}{Lemma}
\newtheorem{remark}{Remark}
\newtheorem{example}{Example}
\newtheorem{theorem}{Theorem}
\newtheorem{definition}{Definition}
\newtheorem{question}{Question}

\xpatchcmd{\proof}{\itshape}{\normalfont\proofnameformat}{}{}
\newcommand{\proofnameformat}{\bfseries}

\newcommand{\notimplies}{\nRightarrow}

%%% prettyref

\usepackage{prettyref}
\newcommand{\pref}[1]{\prettyref{#1}}
\newcommand{\pfref}[1]{Proof of \prettyref{#1}}
\newcommand{\savehyperref}[2]{\texorpdfstring{\hyperref[#1]{#2}}{#2}}
\newrefformat{eq}{\savehyperref{#1}{\textup{(\ref*{#1})}}}
\newrefformat{eqn}{\savehyperref{#1}{Equation~\ref*{#1}}}
\newrefformat{con}{\savehyperref{#1}{Conjecture~\ref*{#1}}}
\newrefformat{lem}{\savehyperref{#1}{Lemma~\ref*{#1}}}
\newrefformat{def}{\savehyperref{#1}{Definition~\ref*{#1}}}
\newrefformat{line}{\savehyperref{#1}{line~\ref*{#1}}}
\newrefformat{thm}{\savehyperref{#1}{Theorem~\ref*{#1}}}
\newrefformat{corr}{\savehyperref{#1}{Corollary~\ref*{#1}}}
\newrefformat{sec}{\savehyperref{#1}{Section~\ref*{#1}}}
\newrefformat{app}{\savehyperref{#1}{Appendix~\ref*{#1}}}
\newrefformat{ass}{\savehyperref{#1}{Assumption~\ref*{#1}}}
\newrefformat{ex}{\savehyperref{#1}{Example~\ref*{#1}}}
\newrefformat{fig}{\savehyperref{#1}{Figure~\ref*{#1}}}
\newrefformat{alg}{\savehyperref{#1}{Algorithm~\ref*{#1}}}
\newrefformat{rem}{\savehyperref{#1}{Remark~\ref*{#1}}}
\newrefformat{conj}{\savehyperref{#1}{Conjecture~\ref*{#1}}}
\newrefformat{prop}{\savehyperref{#1}{Proposition~\ref*{#1}}}
\newrefformat{proto}{\savehyperref{#1}{Protocol~\ref*{#1}}}
\newrefformat{prob}{\savehyperref{#1}{Problem~\ref*{#1}}}
\newrefformat{claim}{\savehyperref{#1}{Claim~\ref*{#1}}}

==> sections/ethics.tex <==
In this Section we will conduct the NeurIPS Ethics Review, a critical and important step in helping ensure beneficial research outcomes. 
The research process of this paper did not cause any direct harm to persons, since our work is theoretical and mathematical, so our ethical analysis focuses on \emph{Societal Impact and Potential Harmful Consequences}. 

The areas of concern on the NeurIPS guidelines for social impact are safety, security, discrimination, surveillance, deception and harassment, environmental, humans rights, and bias and fairness.

Of this list, \emph{discrimination, and bias and fairness} are the most relevant to our work. 
We will consider these notions together.

This section of the Ethics Review directs us to consider `known or anticipated consequences of research.'
The high level idea in our paper is studying and improving the robustness of fairness constrained learning in the presence of malicious noise.
Our work is a step towards models that are robust to malicious noise, which would ideally result in fair \emph{and} accurate learning systems. 
This paper also exposes when models are inevitably fragile, and thus directs actors towards a different solution concept or system.
These two threads would ideally have a positive benefit in mitigating discrimination and bias.

However, there exists a certain constant risk that mathematical models of bias (and models learned on data) are mismatched with
the underlying empirical reality and that when deployed supposedly unambiguously beneficial interventions can be harmful.
The malicious noise model is intentionally a worst case model with quite capacious assumptions, so we believe our results are quite general and would not fall in this trap; but these concerns are worth keeping in mind when considering a new deployment.
In particular, the field of fairness constrained learning needs more experimental verification.

Despite these risks, we thoroughly believe that it is critical to study fairness in learning since different demographic groups exist in the real world  and machine learning can affect those groups differently.  
Theoretical work like ours is critical to exposing fundamental trade-offs and 
baselines that can help craft effective fairness interventions.

We are confident our work passes high ethical standards and is a net ethical benefit to society at large. 

==> sections/intro.tex <==
%\kevin{testedit}
Machine learning continues to be deployed into a wide range of settings and environments including high-stakes decisions, where poor performance can be  harmful to the recipients of a decision. 
%Social contexts infuse many aspects of the data-generation and labeling process, from how the 
%features are distributed across groups, to levels of noise in measuring those features, and to how the labels are assigned to the data-points. 
%This latent social information affecting the data pipeline prompts concerns that learned models may exhibit  disparate performance on some sub-groups, and that by the time this disparity is detected, significant harm could have occurred. 

One way to mitigate or prevent these effects in models is to modify the learning algorithm to include fairness constraints that are evaluated on the training data to result in a `fair'\footnote{Scare quotes here are meant to indicate that many important aspects of fairness are only roughly captured by these group constraints and that group constraints are a relatively weak guarantee.} model.
%These constraints are often thought of a legal or ethical requirement. 
Foundational work showed how several of the constraints \cite{klein16,chouldechova2017fair} are incompatible unless a model has perfect accuracy.

%However,
%as these constraints are often introduced as moral or legal requirements and
%There remain substantial questions about the utility of fairness constrained learning in %deployment. 
In learning theory, fundamental theorems and basic algorithms are typically proven %
and evaluated when assuming an i.i.d training/test set split.
%This simplifies the generalization problem.
%However, 
In the wild, distributions can shift substantially between model development and deployment (e.g. drift over time or due to strategic manipulation) resulting in worse and different performance when a model goes from
training and development to deployment.
%Additionally, where does the disparity in learning come from? 

%Often the disparity can be seen to come from explicit human actions in the past or differing distributions of features. 
%In other ways, the disparity seems to be operationalized as increased uncertainty when making decisions about a subgroup, due to limited or poor quality (e.g. explicitly biased) training data. 

%Collecting better data seems like the gold standard solution, but there may be substantial barriers to that solution.
%In some high stakes contexts, like medical settings, accurate decisions must be made now. 

To capture this concern about learning with unreliable data, we posit that some natural distribution does exist and most of the data does come from this distribution but there is an Adversary who can arbitrarily manipulate some fraction of the available distribution, in order to `fool' the classifier. 

In this malicious noise model, the goal is to learn a classifier with good performance on natural examples and  the fear is that synthetic examples may mislead the learning process. 
Lower bounds in this model typically argue that the malicious noise makes two distributions indistinguishable, so the learner is forced to exhibit high error on one of the two distributions.

Recent work in this adversarial model \cite{lampert}\footnote{Our learning settings are similar, with a key difference using an improper classifier.} 
has studied the question of fairness constrained learning with empirical risk minimization.
At a high level, that work shows that Fairness Constrained Learning will in the worst case return classifiers with $50\%$ errror due to the dependence on the size of the smaller sub-group.
%has the same worst case performance as unconstrained learning when subject to malicious noise, but complicated by dependence on the size of the smaller sub-group. 


In this work, we probe the durability of these negative results by allowing the learner to exhibit a randomized improper classifier, created from hypotheses in a base class, using some kind of black box processing. 
We term this `closure' of a hypothesis class $\mathcal{H}$, $\closure$, in that we are including hypotheses near to $\mathcal{H}$.
In words, for each classifier $h \in \mathcal{H}$, there exists an $h^{'} \in \closure$, parameterized by two parameters $p,q \in [0,1]$.
\begin{align*}
    h^{'} = 
    \begin{cases}
    h(x) \quad 1-p \\
    \Bern(q) \quad \text{otherwise}
    \end{cases}
\end{align*}
In words, larger $p$ means we ignore more of the information in the base classifier and rely on the $\Bern(q)$.

Similarly, to \cite{lampert}, our work emphasizes the relationship between excess accuracy loss, the size of Group $B$, and the amount of corrupted data. More details of our model will come in Section \ref{subsec:closure}. The main technical question we ask here is:
%
\begin{center}
\emph{When a fairness aware ERM-learner is being targeted by an Adversary with malicious noise, by allowing the learner to exhibit a simple improper learning rule, can we exhibit hypotheses that are as robust to malicious noise as an ERM learner who is indifferent to fairness?}
\end{center}
In the rest of the paper, we shall answer this question in the affirmative for some fairness constraints and show constant 
%
%In other words, the classical result \cite{kearns1988learning}
%\subsection{Our Contributions}



We focus on proving the existence of $h^{'} \in \closure$ that satisfies a given fairness constraint and experiences minimal accuracy loss on the natural data distribution. 
%Our proofs are constructive. 
Now we enumerate a hierarchy of fairness constraints and informally conjecture about how much accuracy is lost for each, when subject to $\alpha$ corruption.
%Here are the notions within order of robustness to malicious noise. (Again, here more robustness mean more accuracy on the natural data (despite the malicious noise) while still satisfying a given fairness constraint on biased data).
%In other words, train and select a model using the 

\begin{align*}
\textit{Demographic Parity} \geq Equal Opportunity \geq  Equalized Odds 
\geq Equal Error Rates
\end{align*}

\begin{theorem} \label{thm: zoo}
Now we combine these fairness notions into one location and discuss their error in the presence of $O(\alpha)$ corruptions. 
Observe that from \cite{malnoise}, unconstrained ERM has an unconditional lower bound of $\Omega(\alpha)$.
This is our baseline and we want Fair ERM in the closure model to compete with this.
\begin{enumerate}
    \item Unconstrained ERM excess error $\Theta(\alpha)$ [exhibit $h^{*}$]
    \item Demographic Parity also has accuracy loss at most $\Theta(\alpha)$
    \item Eopp is at worst $\Omega\sqrt{\alpha})$
    \item Equal Error Rates : $\Omega(1)$
       \item Equalized Odds gets error $\min \{ r_A, r_B \}=\Omega(1)$

    \item Calibration has error in the worst case $\Omega(1)$
    \item Mini-Max Fairness has error in the worst case $\Omega(1)$
\end{enumerate}
\end{theorem}

\begin{tabular}{ |p{2.7cm}||p{2.7cm}|p{2.7cm}|p{2.7cm}|p{2.7cm}| }
 \hline
 \multicolumn{5}{|c|}{ Results Summary} \\
 \hline
 Size of Group $B$ & Demographic Parity &  Equal Opportunity & Equal Error Rates & Equalized Odds \\
 \hline
 $ |A|=|B|$  & AF    &AFG&   004  & 420 \\
$|A| > O(\alpha) = |B|$ &   AX  & ALA   &248 & 420\\
 \hline
\end{tabular}



 
 \subsection{Related Work}

 \cite{lampert} study explore the limits of fairness-aware PAC learning within the classic malicious adversary
model of Valiant \citep{valiant}, where the adversary can replace a fraction of the data points with arbitrary data, with full knowledge of the learning algorithm, the data distribution and
the remaining samples. They focus on binary classification with two popular group fairness constraints - demographic parity (Calders et al., 2009) and equal opportunity (Hardt et al., 2016).
First, let us focus on interpreting their results on parity for a bit.





\begin{enumerate}
    \item First they show that learning under this adversarial model is provably impossible in a PAC sense - there is no learning algorithm that can ensure convergence with high probability
to a point on the accuracy-fairness Pareto front on the set of all finite hypothesis spaces, even in the limit of infinite training data.
\item Furthermore, the irreducible excess gap in the fairness measures they study is inversely proportional to the frequency of the rarer of the two protected attributes groups. This makes the robust learning problem especially hard when one of the protected subgroups in the data is underrepresented. 
\item They also show that the adversary can ensure that any learning algorithm will output a classifier that is optimal in terms of accuracy, but exhibits a large amount of unfairness. 
They also show that their hardness results are tight up to constant factors, in terms of the corruption ratio and the protected group frequencies, by proving matching upper bounds.
\end{enumerate}

Note that this group fairness constraints \cite{chouldechova2017fair,klein16, hardt16} are relatively simple to evaluate and provide relatively weak guarantees in contrast to fairness notions in \cite{dwork2012fairness, dwork2021outcome, hebert2018multicalibration}, among others.  
However, despite this weakness,  these group notions are likely to be used as primitive/first cut notions \cite{metricsinpractice}, so continuing to investigate them in parallel to the stronger fairness notions is worthwhile.

\subsection{Black Box Fairness Processing \red{incomplete}}
%move this else where
Our paper can be thought of as a way to black box post-process an existing model, in order to be fair and accurate.
 There is extensive literatue on post processing methods since they 

 Additionally, post processing in the presence of malicious noise is 
%Fair projection \cite{fairprojection}.

==> sections/results.tex <==
\subsection{Closure Model}
\label{subsec:closure}
The key technical contribution of our paper is combining the worst case attacks of the Malicious Model with simple black-box modifications of the original hypothesis class $\mathcal{H}$. This can be thought of a way to smooth out some of the hardness in the lower bounds created by the Adversary. 

\begin{definition}
    Closure Model: Given \red{todo} 
\end{definition}

